Mechanism Design via the Interim Relaxation

We study revenue maximization for agents with additive preferences, subject to downward-closed constraints on the set of feasible allocations. In seminal work, Alaei~\cite{alaei2014bayesian} introduced a powerful multi-to-single agent reduction based on an ex-ante relaxation of the multi-agent problem. This reduction employs a rounding procedure which is an online contention resolution scheme (OCRS) in disguise, a now widely-used method for rounding fractional solutions in online Bayesian and stochastic optimization problems. In this paper, we leverage our vantage point, 10 years after the work of Alaei, with a rich OCRS toolkit and modern approaches to analyzing multi-agent mechanisms; we introduce a general framework for designing non-sequential and sequential multi-agent, revenue-maximizing mechanisms, capturing a wide variety of problems Alaei's framework could not address. Our framework uses an \emph{interim} relaxation, that is rounded to a feasible mechanism using what we call a two-level OCRS, which allows for some structured dependence between the activation of its input elements. For a wide family of constraints, we can construct such schemes using existing OCRSs as a black box; for other constraints, such as knapsack, we construct such schemes from scratch. We demonstrate numerous applications of our framework, including a sequential mechanism that guarantees a $\frac{2e}{e-1} \approx 3.16$ approximation to the optimal revenue for the case of additive agents subject to matroid feasibility constraints. We also show how our framework can be easily extended to multi-parameter procurement auctions, where we provide an OCRS for Stochastic Knapsack that might be of independent interest.

==> Definitions.tex <==
% 2014 written by S V N Vishwanathan (vishy@ucsc.edu)
% 2015 modified by Jiasen Yang (jiaseny@purdue.edu)

\usepackage{enumitem}

\RequirePackage{latexsym}
\RequirePackage{amsmath}
% \RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage[mathscr]{euscript}
\usepackage[margin=1in]{geometry}
\usepackage[hidelinks]{hyperref}

\usepackage{amsthm}
\usepackage{soul}
\usepackage{bbm}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

%\usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
% \usepackage{tikz}
% \def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

\usepackage[linesnumbered,ruled,vlined,noend]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}


\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

\newcommand{\hrulealg}[0]{\vspace{1mm} \hrule \vspace{1mm}}


\usepackage{cleveref}




% bold epsilon & epsilons
\newcommand{\epsb}{\boldsymbol{\epsilon}}
\newcommand{\erla}{\varepsilon_{\texttt{Q}}}
\newcommand{\emdl}{\varepsilon_{\texttt{mdl},p}}
\newcommand{\enq}{\varepsilon_{\texttt{nq},p}}
\newcommand{\enqin}{\varepsilon_{\texttt{nq},\infty}}
\newcommand{\emdlin}{\varepsilon_{\texttt{mdl},\infty}}
%%% Macros for this paper

\newcommand{\opt}{\operatorname{OPT}}
\newcommand{\dbeta}{\Delta\beta}
\newcommand{\dwb}{\Delta\wb}
\newcommand{\relu}{\operatorname{Relu}}
\newcommand{\Ocaltil}{\tilde{\Ocal}}
\newcommand{\Omegatil}{\tilde{\Omega}}
\newcommand{\dkl}{\operatorname{D_{KL}}}
\newcommand{\Lcaltil}{\tilde{\Lcal}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Dhat}{\hat{\mathcal{D}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Mhat}{\hat{\mathcal{M}}}
\newcommand{\Mtilde}{\widetilde{\mathcal{M}}}
\newcommand{\Dtilde}{\widetilde{\mathcal{D}}}
\newcommand{\Qcal}{\mathcal{Q}}

\newcommand{\Rev}{\operatorname{Rev}}


%%%%% Extra 

\newcommand{\Indic}[1]{\mbox{}\mathbbm{1}\{#1\}}
\newcommand{\RoundedDownOne}{$\floor{\Fhat_{z,i}}_{\ell, \delta}$}
\newcommand{\RoundedDownTwo}{$\floor{\Fcal_{z,i}}_{\ell, \delta}$}

\usepackage{color}
\newcommand{\marios}[1]{\textcolor{blue}{Marios: #1}}
\newcommand{\alex}[1]{\textcolor{red}{Alex: #1}}

%%%%%%

\newcommand{\ex}{\mathbb{E}}
\newcommand{\Ex}[1]{\mbox{}\mathbb{E}\left[#1\right]}
\newcommand{\EX}[2]{\mbox{}\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Var}[1]{\mbox{}\textup{Var}\left(#1\right)}
\newcommand{\Cov}[1]{\mbox{}\textup{Cov}\left(#1\right)}
\newcommand{\Tr}[1]{\mbox{}\textup{tr}\left(#1\right)}
\newcommand{\Trsq}[1]{\mbox{}\textup{tr}^2\left(#1\right)}
% \newcommand{\pr}{\mathbb{P}}
\newcommand{\kl}[2]{\mbox{}\mathbb{KL}\left(#1\,||\,#2\right)}
\newcommand{\tAb}{\widetilde{\Ab}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\ts}{\mathsf{T}}
% \newcommand{\ts}{\top}
% \newcommand{\ind}[1]{\mathbb{I}\{#1\}}
\newcommand{\ind}[1]{\mathds{1}\{#1\}}
\newcommand{\nnz}[1]{\mathsf{nnz}(#1)}
\newcommand{\Diag}[1]{\diag \left\{#1\right\}} % pseudoinverse
\newcommand{\Pinv}[1]{\mbox{}\left(#1\right)^{\dagger}} % pseudoinverse
\newcommand{\inv}[1]{\mbox{}\left(#1\right)^{-1}} % pseudoinverse
\newcommand{\RR}[2]{\mathbb{R}^{#1 \times #2}} % Real numbers
\newcommand{\R}{\mathbb{R}} % Real numbers
\newcommand{\Sqrt}[1]{#1^{\nicefrac{1}{2}}} % pseudoinverse
\newcommand{\defeq}{\triangleq}
% \newcommand{\var}{\text{var}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\todo}[1]{\textcolor{red}{\texttt{TODO}: \emph{#1}}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cbb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

% \newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Abtil}{\widetilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{\Fcal}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}

\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}

\newcommand{\Ascrb}{\boldsymbol{\Ascr}}
\newcommand{\Bscrb}{\boldsymbol{\Bscr}}
\newcommand{\Cscrb}{\boldsymbol{\Cscr}}
\newcommand{\Dscrb}{\boldsymbol{\Dscr}}
\newcommand{\Escrb}{\boldsymbol{\Escr}}
\newcommand{\Fscrb}{\boldsymbol{\Fscr}}
\newcommand{\Gscrb}{\boldsymbol{\Gscr}}
\newcommand{\Hscrb}{\boldsymbol{\Hscr}}
\newcommand{\Iscrb}{\boldsymbol{\Iscr}}
\newcommand{\Jscrb}{\boldsymbol{\Jscr}}
\newcommand{\Kscrb}{\boldsymbol{\Kscr}}
\newcommand{\Lscrb}{\boldsymbol{\Lscr}}
\newcommand{\Mscrb}{\boldsymbol{\Mscr}}
\newcommand{\Nscrb}{\boldsymbol{\Nscr}}
\newcommand{\Oscrb}{\boldsymbol{\Oscr}}
\newcommand{\Pscrb}{\boldsymbol{\Pscr}}
\newcommand{\Qscrb}{\boldsymbol{\Qscr}}
\newcommand{\Rscrb}{\boldsymbol{\Rscr}}
\newcommand{\Sscrb}{\boldsymbol{\Sscr}}
\newcommand{\Tscrb}{\boldsymbol{\Tscr}}
\newcommand{\Uscrb}{\boldsymbol{\Uscr}}
\newcommand{\Vscrb}{\boldsymbol{\Vscr}}
\newcommand{\Wscrb}{\boldsymbol{\Wscr}}
\newcommand{\Xscrb}{\boldsymbol{\Xscr}}
\newcommand{\Xscrbh}{\hat{\Xscrb}}
\newcommand{\Yscrb}{\boldsymbol{\Yscr}}
\newcommand{\Zscrb}{\boldsymbol{\Zscr}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}

\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}

\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

%\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}
\newcommand{\Lmat}{\Lb}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}

\newcommand{\vol}{\text{vol}}



%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathop{\mathbb{E}}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
%\newcommand{\PP}{\mathop{\mathbb{P}}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
% \newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
% \newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\cf}{\emph{cf.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
% \newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{\mathbf{\Theta}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\Lambdab}{\mathbf{\Lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}
\newcommand{\Phib}{\boldsymbol{\Phi}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\hWb}{\widehat{\Wb}}
% \newcommand{\Sreg}{\Sigmab_\mathsf{reg}}
\newcommand{\Sreg}{\widetilde{\Sigmab}}



%-----------------------------
% Palma's commands 
\newcommand{\agniva}[1]{\textcolor{ForestGreen}{[Agniva: #1]}}
\newcommand{\palma}[1]{\textcolor{blue}{[Palma: #1]}}
\newcommand{\haim}[1]{\textcolor{red}{[Haim: #1]}}
\newcommand{\bl}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}

\newcommand{\dimone}{m}
\newcommand{\dimtwo}{n}

\newcommand{\sig}{\sigma}
\newcommand{\sigmin}{\underline{\sigma}}
\newcommand{\sigmax}{\overline{\sigma}}

%\newcommand{\alphatil}{\tilde{\alpha}} // already above
\newcommand{\alphabar}{\bar{\alpha}}

\newcommand{\neigh}{\mathcal{N}(\gamma)}


\newcommand{\Delx}{\Delta \xb}
\newcommand{\Dels}{\Delta \sbb}
\newcommand{\Dely}{\Delta \yb}

\newcommand{\xnew}{\xb(\alpha)}
\newcommand{\snew}{\sbb(\alpha)}
\newcommand{\ynew}{\yb(\alpha)}
\newcommand{\munew}{\mu(\alpha)}
\newcommand{\rnew}{r(\alpha)}

\newcommand{\delxdels}{\hat{\Delta \xb} \circ \hat{\Delta \sbb} }
\newcommand{\delxTdels}{\hat{\Delta\xb}^\ts \hat{\Delta \sbb} }
\newcommand{\xcircs}{\xb \circ \sbb }
\newcommand{\delxdelsnorm}{\|\hat{\Delta \xb} \circ \hat{\Delta \sbb} \|_\infty}

\newcommand{\threefac}{\gamma \sig \mu}
\newcommand{\vTen}{\vb^\ts \one_\dimtwo / \dimtwo}
\newcommand{\vTenfrac}{\frac{\vb^\ts \one_\dimtwo}{\dimtwo}}

\newcommand{\alphamax}{\tilde{\alpha}}
\newcommand{\alphaused}{\bar{\alpha}}

\newcommand{\fapprox}{\tilde{f}}

\newcommand{\factorone}{B}
\newcommand{\factortwo}{A}


%----------------------------
% Experiments 
\newcommand{\tolCG}[0]{$\emph{tolCG}$} % 
\newcommand{\tolOuterRes}[0]{$\tau$}

\newcommand{\precNormal}[0]{$\Qb^{-\nicefrac{1}{2}}\Ab\Db^2\Ab^\ts\Qb^{-\nicefrac{1}{2}}$}

\newcommand{\kprecNormal}[0]{$\kappa(\Qb^{-\nicefrac{1}{2}}\Ab\Db^2\Ab^\ts\Qb^{-\nicefrac{1}{2}}$)}

\newcommand{\Alloc}{\mathcal{A}}
\newcommand{\EW}{\mathcal{EW}}
\newcommand{\SW}{\mathcal{SW}}
\newcommand{\NSW}{\mathcal{NSW}}

\newtheorem{theorem}{Theorem}
\newtheorem{application}{Application}
\newtheorem{theorem*}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{example}{Example}


\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


==> notes.tex <==
\section{FedEx Problem Definition}


We will have $n$ bidders whose types will be of the form (value, deadline) (i.e. $t_i=(v_i,d_i)$). We will assume that for each bidder there are a total of $c$ different possible valuations. We will have one item and a total of $m$ possible shipping dates. Our goal will be to compute the optimal mechanism that consists of an allocation and a payment rule. $\alpha_{i,j}(t)$ will represent the probability that bidder $i$ receives the item at day $j$ when reported types are $t$. $p_i(t)$ represents the payment of bidder $i$ when reported types are $t$. We will assume additive quasi-linear bidders. The utility of a bidder when his true type is $t_i=(v_i,d_i)$ but he reports $t'_i=(v'_i,d'_i)$ and the reported types of the rest of the bidders are $t_{-i}$ is:

\begin{equation*}
    u_i(t_i|t'_i, t_{-i}) = v \cdot \sum^{d_i}_{j=1} \alpha_{i,j}(t'_i, t_{-i}) - p_i(t'_i, t_{-i})  
\end{equation*}

We assume that for each bidder $i$ there exists a prior distribution $\Dcal_i$ from which his value and deadline are drawn. We let values and deadlines be arbitrarily correlated. Let $q_{i,j}$ be the probability that bidder $i$ has deadline $j$ (i.e. $q_{i,j} = \PP_{(v,d) \sim \Dcal_i}[d=j]$). We assume that for each deadline $j$ there exists a marginal distribution function of values $F_{i,j}(x) = \PP_{(v,d) \sim \Dcal_i}[v \le x| d = j]$. Let $f_{i,j}(x)$ be the derivative of $F_{i,j}(x)$

A mechanism is BIC if for every bidder $i$, type $t_i=(v_i,d_i)$ and possible misreport $t'_i=(v'_i,d'_i)$ we have that:

\begin{equation*}
    \EE_{t_{-i} \sim F_{-i}}[u_i(t_i|t_i, t_{-i})] \ge \EE_{t_{-i} \sim F_{-i}}[u_i(t_i|t'_i, t_{-i})]
\end{equation*}

A mechanism is ex-interim IR when $\EE_{t_{-i} \sim F_{-i}}[u_i(t_i|t_i, t_{-i})] \ge 0$.

\section{Equivalent LP}

We will consider the following LP that is equivalent to the FedEx problem described above. Essentially we will assume a different item for each possible delivery date. For each bidder, the valuations of the $m$ different item will be correlated. Assuming a bidder has type $t = (v,d)$ then item $1, \cdots, d$ will all have value $v$ and the rest will have value 0. It is essentially like considering $m$ different levels of service where the bidder has a different valuation for each possible level of service. We will only need to add an extra feasibility constraint where only one item can be allocated. More precisely we have the following LP:


\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{t} \PP[t] \displaystyle\sum\limits_{i \in [n]} p_i(t)\\
\\
\text{s.t.}& \EE_{t_{-i}}\left[\sum_{j} t_{i,j}\alpha_{i,j}(t_i,t_{-i}) - p_i(t_i,t_{-i}) \right] \ge \\ 
&\EE_{t_{-i}}\left[\sum_{j} t_{i,j}\alpha_{i,j}(t'_i,t_{-i}) - p_i(t'_i,t_{-i}) \right] \hspace{1 cm} & \forall i\in [n], t_i, t'_i \\ 
\\
&  \EE_{t_{-i}}\left[\sum_{j} t_{i,j}\alpha_{i,j}(t_i,t_{-i}) - p_i(t_i,t_{-i}) \right] \ge 0 & \forall i\in [n], t_i \\

\\
& \displaystyle\sum\limits_{i \in [n]} \displaystyle\sum\limits_{j \in [m]} \alpha_{i,j}(t) \le 1 & \forall t \\
& \alpha_{i,j}(t) \ge 0 & \forall i \in [n], j \in [m], t 
\end{array}
\end{equation*}

\section{Applying the CDW framework}

Most things that we will need here are already proven Cai et al. \cite{CDW_2}. Here I will present the high-level intuition and will go into more detail when necessary.

Let's call $\Fcal$ the set of feasible allocation rules and $F(\Fcal, \Dcal)$ the set of feasible interim allocation rules when values are drawn from $\Dcal$. Let $f_i$ be a function that maps types to virtual types and $VVCG_{\Fcal}(\{f_i\}_{i \in [n]})$ be the VCG mechanism when run with virtual values $\{f_i\}_{i \in [n]}$ and feasibility constraints $\Fcal$. For ease of notation let $\vec{w} \in \R^{m \cdot c}$ be a vector such that for any bidder $i$ and possible type $t_i$, we have $w_{i,j} = f_{i,j}(t_i) \cdot \PP[t_i]$. Under this notation  $VVCG_{\Fcal}(\vec{w})$ represents $VVCG_{\Fcal}(\{f_i\}_{i \in [n]})$.

\begin{theorem}[Theorem 1 \cite{CDW_2}]
    Let $\Fcal$ be any set system of feasibility constraints, and $\Dcal$ be nay (possibly correlated) distribution over bidder types with finite support. Then every feasible reduced form (with respect to $\Dcal$) can be implemented as a distribution over at most $m \cdot n \cdot c+1$ simple virtual VCG allocation rules. \footnote{We call a VCG allocation simple if it has a unique max-weight allocation.}
\end{theorem}

We first re-write our LP using the interim allocation and payment rules. We also require our interim allocation rule $\pi$ to be in the feasible set $F(\Fcal, \Dcal)$. Recall that in our setting an interim allocation rule $\pi$ is in $F(\Fcal, \Dcal)$ if it is induced by an allocation rule that only allocates one item. 

\begin{proposition}[Proposition 1 \cite{CDW_2}]
    If $|\Dcal|$ is finite, $F(\Fcal, \Dcal)$ is a convex polytope.
\end{proposition}

\begin{lemma}[Lemma 1 \cite{CDW_2}]
   Let $\vec{\pi}$ be the reduced form of mechanism $VVCG_{\Fcal}(\vec{w})$ (with an arbitrary tie-breaking rule) when bidders are sampled from $\Dcal$. Then for all $\vec{\pi'} \in F(\Fcal, \Dcal)$, $\vec{\pi} \cdot \vec{w} \ge \vec{\pi'} \cdot \vec{w}$. 
\end{lemma}

\begin{proposition}[Proposition 2 \cite{CDW_2}]
    Every corner of $F(\Fcal, \Dcal)$ can be implemented by a simple virtual VCG allocation rule, and the reduced form of any simple virtual VCG allocation rule is a corner of $F(\Fcal, \Dcal)$.
\end{proposition}

 Now let $W_{\Fcal}(\vec{w})$ be the total expected weight of items allocated by $VVCG_{\Fcal}(\vec{w})$. 
 
 \begin{corollary}[Corollary 1 \cite{CDW_2}]
    A reduced form $\vec{\pi}$ is feasible (with respect to $\Fcal$ and $\Dcal$) if and only if, for any $\vec{w} \in [-1,1]^{n \cdot m \cdot c}$ it holds that $\vec{\pi}\vec{w} \le W_{\Fcal}(\vec{w})$.     
 \end{corollary}

Cai et. al. \cite{CDW_2} also provide a way to implement tie-breaking rules by modifying $\vec{w}$ to $\Vec{w}'$ without any loss to the objective. This tie-breaking rule ensures that the VCG mechanisms that will arise will be simple. For simplicity, we will assume from now on that ties do not occur since we can eliminate them using their analysis.

Now we will try to create an efficiently computable separation oracle for our reduced form LP. Consider the following function: $g_{\vec{\pi}}(\vec{w}) = W_{\Fcal}(\vec{w}) - \vec{\pi}\vec{w}$. Given some candidate interim allocation rule $\vec{\pi}$ we would like to minimize $g_{\vec{\pi}}(\vec{w})$. If this minimum is non-negative then our candidate interim allocation rule is feasible. If it is negative then it is infeasible and the minimizing weights $\vec{w}$ give us the separating hyperplane. Thus we write the following LP:

\begin{equation*}
\begin{array}{ll@{}ll}
\text{minimize}  & t - \vec{w} \cdot \vec{\pi}\\
\\
\text{s.t.}& t \ge \vec{x} \cdot \vec{w} \hspace{25pt}&\forall \vec{x} \in F(\Fcal, \Dcal)
\end{array}
\end{equation*}

To solve this LP we will use an internal separation oracle, which given some $t, \vec{w}$ will determine whether there exists an $\vec{x} \in F(\Fcal, \Dcal)$ such that $t \le \vec{x} \cdot \vec{w}$. However, if there exists such $\vec{x}$ then for sure the interim allocation rule of $VVCG_{\Fcal}(\vec{w})$ also violates the constraint. Thus our problem boils down to calculating the interim allocation rule of $VVCG_{\Fcal}(\vec{w})$ in polynomial time. One way of doing this is by sampling types from $\Dcal$ in a specific way which in turn allows us to show that $F(\Fcal, \Dcal)$ and $F(\Fcal, \Dcal')$ are close with high probability (where $\Dcal'$ is the empirical distribution). Fortunately, our setup allows us to do something better and easier.

Since we only allocate one item, a bidder gets the item if he has the highest virtual value. For every bidder and possible type, we simply need to calculate the probability that all other bidders have smaller virtual types than him. We can "brute force" this in time polynomial in $c,n, m$ and calculate exactly the interim allocation rule of $VVCG_{\Fcal}(\vec{w})$.

The only thing left now to do is construct a corner oracle.\footnote{A corner oracle takes as input a polytope $P$ and $k$ hyperplanes $H_1, \cdots, H_k$. If no hyperplane intersects $P$ in its interior and there is a corner of $P$ in all hyperplanes then such corner is output (otherwise the behavior can be arbitrary)} Using the separation oracle we have described above with the corner oracle we can decompose any feasible interim allocation rule as a linear combination of $VVCG$ mechanisms.

\begin{theorem}[Theorem 13 \cite{CDW_1}]
    Let $P$ be a $d$-dimensional polytope with corner oracle CO and separation oracle SO such that each coefficient of every hyperplane ever output by SO is a rational number of bit complexity $b$. Then there is an algorithm that decomposes any point $\vec{x} \in P$ into a convex combination of at most $d+1$ corners of $P$. Furthermore, if $\ell$ is the maximum number of bits needed to represent a coordinate of $\vec{x}$, then the runtime is polynomial in $d, b, \ell$ and the runtimes of SO and CO on inputs of bit complexity $poly(d,b\ell)$
\end{theorem}

Our corner oracle works as follows:
\begin{itemize}
    \item Input: $k$ hyperplanes in the form $(\vec{w_1}, h_1), \cdots, (\vec{w_k}, h_k)$
    \item set $\vec{w} = \sum^k_{i=1} \frac{1}{k}\vec{w_i}$
    \item output the reduced form of $VVCG_{\Fcal}(\vec{w})$
\end{itemize}

\begin{theorem}[Theorem 3 \cite{CDW_2}]
    The Corner Oracle described by the above procedure correctly outputs a corner of $F(\Fcal, \Dcal)$ contained in $\cap_{j=1}^k H_j$ whenever the corresponding hyperplanes are boundary hyperplanes of $F(\Fcal, \Dcal)$ and $\cap_{j=1}^k H_j$ contains a corner. 
\end{theorem}

The above ideas fully describe how to get an FPTAS for the multi-bidder FedEx problem. If we had directly used the ideas we would have ended up with an FPRAS however the specific constraints of our problem helped us produce something strictly better. The runtime of the algorithms presented depend also on the bit complexity of our inputs. For ease of exposition, we have abstracted those technicalities. For a more detailed approach consult \cite{CDW_2}. The above idea generalizes naturally also for multi-item FedEx problems, however, I presented here the single item for ease of exposition.

\newpage
\section{Rich-Ad Auctions with ex-post Budgets}


There exists a set $\Ncal$ of $n$ advertisers (bidders) and a universe of rich ads $\Scal$. Each advertiser $i \in \Ncal$ has a private value per click $v_i$ and a private set of rich ads $A_i \subseteq \Scal$. For every advertiser $i \in \Ncal$ and each rich ad $j \in \Scal$ has a publicly known space $w_{i,j}$ and a publicly known click-through rate $c_{i,j}$. If advertisement $j \notin A_i$, then the value of advertiser $i$ for that advertisement is $v_{i,j} = 0$, otherwise it is $v_{i,j} = c_{i,j} \cdot v_{i}$. An allocation $x \in [0,1]^{n \times |\Scal|}$ indicates the probability $x_{i,j}$ that ad $j$ is allocated to advertiser $i$. A payment $p_i \in \R^{n}$ indicates the amount $p_i$ that advertiser $i$ has to pay the auctioneer. We will have the following constraints. We can allocate at most one ad per advertiser (i.e. $\sum_{j \in \Scal} x_{i,j} \le 1$ for all $i \in \Ncal$). Also, the total space used can be at most $W$ (i.e. $\sum_{i \in \Ncal} \sum_{j \in \Scal} x_{i,j} w_{i,j} \le W$). Furthermore, for each advertiser $i$ there exists a budget $b_i$ which means that bidder $i$ cannot pay more than $b_i$ to the auctioneer. We assume that for each bidder $i$ there exists a prior distribution $\Dcal_i$ from which his value per click and private set are drawn. We will assume that there exists an ordering of the different ads. If a bidder $i$ has ad $j$ (i.e. $j \in A_i$), then he also has every ad $j'$ such that $j' \le j$ in his private set (i.e. $j' \in A_i: j' \le j$). Let $q_{i,j}$ be the probability that bidder $i$ has private set $\Acal = \{j': j' \le j, j' \in \Scal\}$. We assume that for each such set, there exists a marginal distribution function of values $F_{i,j}(x) = \PP_{(v,j') \sim \Dcal_i}[v \le x| j = j']$. Let $f_{i,j}(x)$ be the derivative of $F_{i,j}(x)$. We want to design a BIC and ex-post IR mechanism. Our goal will be to maximize the expected revenue of our mechanism. If $c$ is the number of possible values per click and $m$ the cardinality $\Scal$ (i.e. $m = |\Scal|$) the cardinality of the set of possible types is $c \cdot m$ which is polynomial to our input size. If we do not care about ex-post budget constraints and we can allow fractional (i.e. randomized) allocations then we can solve this problem using the ideas developed above for the FedEx problem. 

\section{Reducing Rich-Ads to Algorithmic Design}

Consider the following general Bayesian Mechanism Design problem:

\vspace{5pt}
\noindent
\textbf{BMeD($\Fcal, \Vcal, \Ocal$):} \\
\textit{Input:} For each bidder $i \in [n]$, a finite set $T_i \subseteq \Vcal$, and a distribution $\Dcal_i$ over $T_i$, presented by explicitly listing all types in $T_i$ and their corresponding probability. \\
\textit{Output:} A feasible (selects an allocation in $\Fcal$ with probability 1), BIC, (interim) IR mechanism for bidders drawn from $\Dcal = \times_{i \in [n]} \Dcal_i$. \\
\textit{Goal:} Find a mechanism that optimizes $\Ocal$ in expectation, with respect to our constraints (when bidders with types drawn from $\Dcal$ play truthfully). \\
\textit{Approximation:} An algorithm is said to be an $(\varepsilon, \alpha)$-approximation if it finds an $\varepsilon$-BIC mechanism whose expected value of $\Ocal$ is at least $\alpha \cdot OPT - \varepsilon$. 
\vspace{5pt}

Due to the work of Cai et. al. \cite{CDW_4} we know that an $(\varepsilon, \alpha)$-approximation to the \textbf{BMeD($\Fcal, \Vcal, \Ocal$)} problem can be efficiently computed given black-box access to a $\alpha$-approximation poly-time algorithm for a generalized objective optimization problem denoted by \textbf{GOOP($\Fcal, \Vcal, \Ocal$)}.

\vspace{5pt}
\noindent
\textbf{GOOP($\Fcal, \Vcal, \Ocal$):} \\
\textit{Input:} For each $i \in [n]$ a type $t_i \in \Vcal$, multiplier $m_i \in \R$, and virtual valuation function $g_i \in \Vcal ^{\times}$ (where $\Vcal ^{\times}$ denotes the closure of $\Vcal$ under addition and (possibly negative) scalar multiplications). \\
\textit{Output:} An allocation $x \in \Fcal$ and payments $p \in \R^{n}_{+}$. \\
\textit{Goal:} Find $\argmax_{x \in \Fcal, p} \left\{ \Ocal(t, x, p) + \sum_{i \in [n]} m_i \cdot p_i + \sum_{i \in [n]} g_i(x)  \right\}$ \\
\textit{Approximation:} $(x^*, p^*)$ is said to be an $\alpha$-approximation if $ \Ocal(t, x^*, p^*) + \sum_{i \in [n]} m_i \cdot p^*_i + \sum_{i \in [n]} g_i(x^*)  \ge \alpha \cdot \argmax_{x \in \Fcal, p} \left\{ \Ocal(t, x, p) + \sum_{i \in [n]} m_i \cdot p_i + \sum_{i \in [n]} g_i(x)  \right\}$. 
\vspace{5pt}

More formally we have the following theorem:

\begin{theorem}[Theorem 4 \cite{CDW_4}]
    For all $\Fcal, \Vcal, \Ocal$, and $\varepsilon > 0$, if there is a poly-time $\alpha$-approximation algorithm $G$, for \textbf{GOOP($\Fcal, \Vcal, \Ocal$)}, there is a poly-time $(\varepsilon, \alpha)$-approximation algorithm for \textbf{BMeD($\Fcal, \Vcal, \Ocal$)} as well. Specifically, if $\ell$ denotes the input length of a \textbf{BMeD($\Fcal, \Vcal, \Ocal$)} instance, the algorithms runs in time poly($\ell, 1/\varepsilon$), makes poly($\ell, 1/\varepsilon$) black box calls to $G$ on inputs of size poly($\ell, 1/\varepsilon$), and succeeds with probability $1-exp(-poly(\lambda, 1/ \varepsilon))$ 
\end{theorem}

Our main issue is that \textbf{BMeD($\Fcal, \Vcal, \Ocal$)} does not accommodate for ex-post IR and ex-post budget constraints. We will do the following: we will not optimize for revenue but we will optimize for the following ``custom made'' function. Let $\Ocal(v, b, x, p) = \sum_{i \in [n]} p_i$, if $0 \le p_i \le \min\{b_i, \sum_{j \in A_i} x_{i,j} \cdot \alpha_{i,j} \cdot v_i\}$, otherwise $\Ocal(v, b, x, p) = -\infty$. This function was used by Daskalakis et. al. \cite{CDW_5} to accommodate for ex-post IR and ex-post budget constraints. It is easy to see that the objective function is concave and thus we can use the aforementioned reduction. We end up with the following Rich-Ad Algorithmic Problem:

\vspace{5pt}
\noindent
\textbf{RAAP:} \\
\textit{Input:} For each $i \in [n]$ a private set of rich ads $A_i$, a value per click $v_i$, budget $b_i$, for each ad $j \in \Scal$ a space $w_{i,j}$, and a click-through rate $\alpha_{i,j}$. We are also given an upper bound on the total length $W$. Finally, we are given price multipliers $m_i \in \R$ and virtual values $g_{i,j} \in \R$ for all $i \in [n], j \in \Scal$.\\
\textit{Output:} An allocation $x \in \{0,1\}^{m,n}$ and price $p$ such that $\sum_{j \in \Scal} x_{i,j} \le 1$ for all $i$ (each advertiser gets at most one ad), $\sum_{j \in A_i} x_{i,j} \cdot \alpha_{i,j} \cdot v_i \ge p_i$ (ex-post IR), $p_i \le b_i$ (ex-post budget respecting), $p_i \ge 0$, and $\sum_{i \in [n]} \sum_{j \in \Scal} x_{i,j} \cdot w_{i,j} \le W$ (ex-post space constraint). \\
\textit{Goal:} Find $\argmax_{x,p} \{\sum_{i \in [n]} m_i \cdot p_i + \sum_{i \in [n]} \sum_{j \in \Scal} x_{i,j} \cdot g_{i,j}\}$ (virtual revenue plus virtual welfare). 
\vspace{5pt}

If our integral solution to \textbf{RAAP} is an $\alpha$-approximation to the fractional one then given the reduction of Cai et. al. \cite{CDW_4} we will have an algorithm that computes an $(\varepsilon, \alpha)$-approximation to the rich ad auction mechanism design problem.

Now that we have introduced the knapsack constraint there might exist an arbitrarily big integrality gap. Consider the following instance. There is only one rich ad and all advertisers have it in their set of rich ads. The space of that ad is $w$ and the upper bound on the space is $w=W$ (effectively only one bidder will get advertised due to that constraint). Every bidder $i$ has the same hard budget constraint $b_i=b$, and also $v_i \cdot a_{i,1} = n \cdot b$. Finally let all $g_{i,j} = 0$ and all $m_i = 1$. It is clear to see that any integral solution will achieve a virtual objective of $b$ since only one bidder can get advertised and his payment can be at most $b$ (and everybody else's payment will be 0). Now consider the following fractional solution. Every bidder gets $x_{i,1}=\frac{1}{n}$. This allows us to charge everyone $p_i = b$ achieving a total virtual objective of $n \cdot b$. This example demonstrates that there is an arbitrarily big integrality gap (between the optimal integral and fractional solution) given these constraints. On the other hand, if we allow for fractional solutions then our problem becomes much easier since we can express \textbf{RAAP} as a polynomially sized LP. 

\section{Solving Unit-Demand bidders with knapsack constraints using OCRS}

Consider a little bit different setting than the Rich-ads outlined earlier. We have $m$ different ads and the valuation of each ad $j \in [m]$ for each bidder $i \in [n]$ follows some distribution $\D_{i,j}$. The valuation of each add is drawn independently. Bidders are unit demand and all ads have some weight $w_j$. Our goal is to find the revenue maximizing mechanism were the total weight of items sold cannot exceed some total weight $W$. We will show how to find a simple and approximately optimal solution using the OCRS framework developed by Feldman et. al. \cite{Feldman2021OCRS}. 

We first relax our problem by considering the copies setting introduced by Chawla et. al. \cite{Shuchi2010Copies}. For each combination of ad $j$, bidder $i$ we will have a new copy of that ad and a copy of that bidder. The new bidder (copy) will only be interested in the corresponding new add (copy) with a valuation that is drawn form $\D_{i,j}$. We will have the knapsack feasibility constraint and the matroid constraint that only one copy of each bidder can win an item. Since our original bidders are unit demand this is a relaxation of our original problem. Since this is a single dimensional setting we can find the optimal mechanism using Myerson. Lets say that in Myersons optimal mechanism, gives copy $(i,j)$ the corresponding ad with probability $x_{i,j}$. Assuming regular distributions (if not then we need to iron the distributions) for each copy we can set the maximum price $p_{i,j}$ such that $\PP_{v \sim \D_{i,j}}[v \ge p_{i,j}]=x_{i,j}$. This posted price mechanism yields more revenue than Myersons mechanism we calculated earlier. The only issue is that based on the realizations of the random valuations, the final outcome might not be feasible. A key observation though is that our fractional algorithm is within the feasible polytope. That is why we can use the OCRS framework to come up with a sequential posted price mechanism that is always feasible and makes on expectation at least a constant fraction of our relaxations revenue. Since the mechanism we will come up with will work for any adversarial order in which copies arrive, it will also work for the sequence where all the copies of the bidder arrive together and the original bidder chooses the order i n which his copies arrive. Thus the mechanism will also work for our original bidders.

First, lets give some background on OCRSs. Consider a finite ground set $N = \{e_1, \cdots , e_n\}$ and a family of feasible subsets $\Fcal \subseteq 2^N$, which is down-closed. Let $P_{\Fcal}$ be the convex hull of all characteristic vectors of feasible sets. 

\begin{definition}[Definition 1.2 \cite{Feldman2021OCRS}, OCRS]
    Let us consider the following online selection setting. A point $x \in P$ is given, and let $R(x)$ be a random subset of active elements such that every element $e \in N$ belongs to $R(x)$ with probability $x_e$, independently. The elements $e \in N$ reveal one by one whether they are active (i.e., $e \in R(x)$), and the decision whether to select an active element has to be taken irrevocably before the next element is revealed. An OCRS for $P$ is an online algorithm that selects a subset $I \subseteq R(x)$ such that $1_I \in P$.
\end{definition}

\begin{definition}[Definition 1.4 \cite{Feldman2021OCRS}, greedy OCRS]
    Let $P \subseteq [0,1]^N$ be a relaxation for the feasible sets $\Fcal \subseteq 2^N$. A greedy OCRS $\pi$ for $P$ is an OCRS that for any $x \in P$ defines a down-closed subfamily of feasible sets $\Fcal_{\pi, x} \subseteq \Fcal$, and an element $e$ is selected when it arrives if, together with the already selected elements, the obtained set is in $\Fcal_{\pi, x}$.
    
    If the choice of $\Fcal_{\pi, x}$ given $x$ is randomized, we talk about a randomized greedy OCRS; otherwise, we talk about a deterministic greedy OCRS. We also simplify notation and abbreviate $\Fcal_{\pi, x}$ by $\Fcal_x$ when the OCRS $\pi$ is clear from the context.
\end{definition}

\begin{definition}[Definition 1.6 \cite{Feldman2021OCRS}, c-selectability]
    Let $c \in [0,1]$. A greedy OCRS for $P$ is $c$-selectable if for any $x \in P$ we have:

    \[\PP[I \cup \{e\} \in  \Fcal_{x} \forall I \subseteq R(x), I \in \Fcal_x] \ge c, \: \forall e \in N \]
\end{definition}

\begin{definition}[Definition 1.8 \cite{Feldman2021OCRS}, (b,c)-selectability]
    Let $b,c \in [0,1]$. A greedy OCRS for $P$ is $(b,c)$-selectable if for any $x \in b \cdot P$ we have:

    \[\PP[I \cup \{e\} \in  \Fcal_{x} \forall I \subseteq R(x), I \in \Fcal_x] \ge c, \: \forall e \in N \]
\end{definition}

Where in the above definition $b \cdot P$ is the polytope $P$ shrunk by a factor of $b$.

\begin{theorem}[Theorem 1.11 \cite{Feldman2021OCRS}]
    There exist the following:
    \begin{itemize}
        \item For every $b \in [0,1]$, a $(b, 1-b)$-selectable deterministic greedy OCRS for matroid polytopes.
        \item For every $b \in [0,1]$, a $(b, e^{-2b})$-selectable deterministic greedy OCRS for matching polytopes.
        \item For every $b \in [0,1]$, a $(b, \frac{1-2b}{2-2b})$-selectable randomized greedy OCRS for knapsack polytopes.
    \end{itemize}
\end{theorem}

\begin{theorem}[Theorem 1.12 \cite{Feldman2021OCRS}]
    If $\pi^1$ is a $(b, c_1)$-selectable greedy OCRS for a polytope $P_1$, and $\pi^2$ is a $(b, c_2)$-selectable greedy OCRS for a polytope $P_2$, then there exists a $(b, c_1 \cdot  c_2)$-selectable greedy OCRS for the polytope $P_1 \cap P_2$ which is efficient if $\pi^1$, $\pi^2$ are.
\end{theorem}

In our setting we have a knapsack and a matroid constraint. Thus, there exists a greedy $(b, (1-b)\cdot \frac{1-2b}{2-2b})$. For $b=1/4$ this gives us a $16$-approximation for our problem. We simply consider copies one by one. We consider a copy with probability $b$ (this way we shrink our polytope by $b$) and only if with his selection, and the set of copies we have selected thus far is within $\Fcal_{\pi, x}$. We give the designated posted price $p_{i,j}$ to this copy. By definition of greedy OCRS this process works for any adversarial order of arrivals and is a $16$-approximation for our relaxed problem. Thus the outlined procedure is a simple sequential posted price mechanism that yields a $16$-approximation for our problem.

\section{Simple mechanism for rich-ads using CDW}


Using the CDW framework (\cite{CDW_1}, \cite{CDW_2}, \cite{CDW_3}, \cite{CDW_4}, \cite{CDW_5}) we can find the optimal interim allocation rule for our problem. Using this interim allocation rule we can compute the expected size of items allocated to each bidder.

We consider two settings. The heavy and the light setting. In the heavy setting we only consider the ads $j$ for which $w_j > W/2$. In the light setting we consider only the rest items. It is easy to see that $OPT \le OPT_{light} + OPT_{heavy}$ where $OPT$ is the expected revenue of the optimal mechanism for our original setting, $OPT_{light}$ is the expected revenue of the optimal mechanism for the light setting, and $OPT_{heavy}$ is the expected revenue of the optimal mechanism for the heavy setting. 

Considering the heavy setting we can see that only one add can be allocated. Using CDW framework we can find the probability with which each bidder is beeing served. Let $x_i$ be that probability for bidder $i$. Our mechanism approaches bidders one by one and runs the optimal mechanism for one bidder where he is being served with probability at most $x_i/2$. Each bidder is being considered with probability at least $1/2$ and from each bidder we make on expectation at least $1/2$ the revenue we made from him in the mechanism that CDW produced.\footnote{Although here we do not take into account the size of the items it is not clear what the single bidder optimal mechanism looks like}.

For the light setting we run again the CDW framework to find the expected size of items allocated to each bidder. Let for bidder $i$ this value be $Q_i$. We will approach each bidder sequentially and serve them with a 1/4 probability. For each one we will run the optimal algorithm that gives them an item with expected weight $Q_i$. Let $X_i$ be the random variable that indicates the sum of weights of items given until some specific bidder $i$ in our mechanism. Using Markov's inequality we can see that $\PP[X_i \ge 1/2 \cdot W] \le  \frac{1/4 \cdot \sum_{j \le i} Q_j}{1/2 \cdot W} \le \frac{1/4 \cdot W}{1/2 \cdot W} = 1/2$. Since each add has weight at most $W/2$ (light setting) and we can sell only one add per bidder, the maximum weight that we can ever allocate to one bidder is $W/2$. Thus with probability $1/2$ we will reach an arbitrary bidder and with probability $1/4$ we will select him and run the optimal ,mechanism on him. Thus each bidder is served with a total probability of $1/8$.

\subsection{Which mechanism should we run per bidder?}

The previous analysis relies on running a mechanism per bidder where the revenue extracted by each bidder is comparable to the revenue that is extracted from him in the optimal mechanism. To do so we simply run the CDW framework. This will return an interim allocation ($\pi$) and payment rule ($q$). When we approach a bidder $i$ we ask him his cut off $c$ and valuation per click $v_i$. We give him add $j$ with probability $\pi_{i,j}(c,v_i)$ (i.e. the interim probability with which CDW allocates this item) and we charge him $q_{i}(c, v_i)$. The mechanism is obviously truthful since the mechanism returned from CDW is BIC. The expected revenue per bidder is the same as the CDW framework and the probability with which an item is sold and the expected size of the allocated bundle is the same. The only issue is that since we approach each bidder sequentially the mechanism is ex-ante but not ex-post feasible. To transform this idea into an ex-post feasible mechanism we use the OCRS type analysis we discussed above.

Although each bidder is approach sequentially the mechanism we apply to each bidder is essentially a menu that could be very big. Our next goal should be to leverage the specific properties of our problem to show that we can compute a simple menu that extracts a constant fraction of the per-bidder optimal revenue.

==> old.tex <==

\section{OLD STUFF}

\subsection{Additive bidders.}


\subsubsection{General Framework.}

Assume that we have a set of $m$ items and $n$ bidders. Each bidders valuation is drawn from some known distribution $v_i \sim \Dcal_i$. Also assume that we have some hard constraints on the feasible allocation represented by a polytope $\Fcal \subseteq 2^{mn}$. Now let $P_{\Fcal}$ be the convex hull of all characteristic vectors of $\Fcal$ (i.e. $P_{\Fcal} = conv\{\mathbf{1_{F}}: F \in \Fcal\}$). Also let $P_{\Fcal}^i$ be the polytope that corresponds to bidder $i$ (this is the polytope $P_{\Fcal}$ when we only consider the $m$ dimension that correspond to the allocation of bidder $i$). Now let $\pi$ be the interim allocation rule and $q$ be the interim payment rule. 
For ease of analysis also define $w$ such that $w_{i,j} = \sum_{v_i \in \Vcal_i} \PP[v_i] \cdot \pi_{i,j}(v_i)$. 

%Also let $w^{-i'}$ be the vector such that $w^{-i'}_j = \sum_{i \in [n]-\{i'\}} \sum_{v_i \in \Vcal_i} \PP[v_i] \cdot \pi_{i,j}(v_i)$. 
%We are going to have a series of $k$ high dimensional convex polytopes $\{P_z\}_{z \in [k]}$ such that $\forall z \in [k]: P_z \subseteq P_{\Fcal}$. Also we will have a probability vector $\mathbf{p} \in [0,1]^k$ ($||\mathbf{p}||_1=1$). With probability $p_z$ we are going to do the following. 
We are going to run the following LP:

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{i \in [n]} \displaystyle\sum\limits_{v_i \in \Vcal_i} \PP[v_i] q_i(v_i)\\
\\
\text{s.t.}& \sum_{j} v_{i,j}\pi_{i,j}(v_i) - q_i(v_i) &\ge \sum_{j} v_{i,j}\pi_{i,j}(v'_i) - q_i(v'_i) & \forall i\in [n], v_i, v'_i \in \Vcal_i\\  
\\
&  \sum_{j} v_{i,j}\pi_{i,j}(v_i) - q_i(v_i) &\ge 0 & \forall i\in [n], v_i \in \Vcal_i  \\
\\
& \pi_i(v_i)\in P_{\Fcal}^i && \forall i\in [n], v_i \in \Vcal_i
\\
\\
& w\in P_{\Fcal}
\end{array}
\end{equation*}

Then we are going to approach each bidder sequentially. We will have a set $\{\Fcal_z\}_{z \in [k]}$ feasibility sets such that $\forall z \in [k]: \Fcal_z \subseteq \Fcal$. At the very beginning we are going to choose set $\Fcal_z$ with probability $\lambda_z$. Bidder $i$ will be considered with probability $b$ or skipped with probability $1-b$. The bidders that have not been  considered yet do not know which previous bidders have been skipped or what items the non-skipped bidders received.  We are going to offer bidder $i$ a menu (if he is not skipped) with a total of $|\Vcal_i|$ menu items. The tuples (bidder, item) that are served are going to be added to a set $\Ical$. Once the bidder chooses an menu item we are going to sequentially consider each item $j \in [m]$ in that menu choice, flip a biased coin with probability $\pi_{i,j}(v_i)$, and independently a coin $p_{i,j}(v_i)$. If both outcomes are $1$, then we greedily add it to $\Ical$ as long as $\Ical \cup \{(i,j)\} \in \Fcal_z$. Our objective will be to choose $\{\Fcal_z\}_{z \in [k]}$, $\lambda$, and $p$ in such a way that from the perspective of the bidder he will receive item $j$ with probability exactly $c\pi_{i,j}(v_i)$ if he chooses menu item $v_i$. From the perspective of the bidder the randomness of the mechanism comes from the random selection of $\Fcal_z$, the randomness of the other bidders and the randomness of the coin flips for each item. He then is going to be charged a price of $c \cdot q_i(v_i)$. Notice that due to the constraints of our LP, a bidder whose type is $v_i$, is going to choose menu item $v_i$. Thus, our revenue on expectation is going to be $b \cdot c$ times the revenue suggested by our LP which is a relaxation of the LP that computes the optimal feasible mechanism. Thus our mechanism by construction extracts at least $b \cdot c$ times the optimal revenue. We are going to call such mechanism $(b,c)$-selectable. 

An important note here is that although the above procedure might seem complicated, all the different technical parts are needed only for the analysis of our mechanism. The actual mechanism from the perspective of the bidder will look like a menu with $|\Vcal_i|$ choices and for choice $i$ he is going to receive item $j$ with probability $c\pi_{i,j}(v_i)$ and pay $cq_{i}(v_i)$. This is arguably a simple sequential menu mechanism assuming that $|\Vcal_i|$ is polynomial is size. 


\subsubsection{A Basic Case.}
\label{sec:BasicCase}

The above concept is quite abstract. So lets first see how we can come up with a simple and efficiently computable BIC mechanism where the only constraint is that we can sell each item once. Notice that $P_{\Fcal}$ can be fully characterized by the following set of inequalities $\forall j \in [m] \sum_{i \in [n]} w_{i,j} \le 1$. We will have $\Fcal_1 = \Fcal$ and $\lambda_1=1$.  Let $A_{i,j}$ be the event that item $j$ is still available at bidder $i$'s turn. Lets call $x_{i,j} = \PP[A_{i,j}]$. We will compute $x_{i,j}$ inductively. As our base case we have that $\forall j \in [m], x_{1,j}=1$. We are going to have $p_{i,j}(v_i) = \frac{1}{(1+b)x_{i,j}}$ (we will later show that this is indeed a valid probability). Thus $p_{1,j}(\cdot) = \frac{1}{1+b}$. It is not difficult to see that $x_{i+1,j} = x_{i,j}\cdot\left(1-b+b\sum_{v_i \in \Vcal}\PP[v_i](1-\pi_{i,j}(v_i))+b\sum_{v_i \in \Vcal}\PP[v_i]\pi_{i,j}(v_i)\left(1-\frac{1}{(1+b)x_{i,j}}\right)\right)$. Notice that :

\begin{align*}
    x_{i+1,j} &= x_{i,j}\cdot\left(1-b+b\sum_{v_i \in \Vcal}\PP[v_i](1-\pi_{i,j}(v_i))+b\sum_{v_i \in \Vcal}\PP[v_i]\pi_{i,j}(v_i)\left(1-\frac{1}{(1+b)x_{i,j}}\right)\right)\\
    &= x_{i,j}\cdot\left(1-b+b(1-w_{i,j})+bw_{i,j}\left(1-\frac{1}{(1+b)x_{i,j}}\right)\right)\\
    &= x_{i,j}\cdot\left(1-w_{i,j}\frac{b}{(1+b)x_{i,j}} \right)\\
    &= x_{i,j} - w_{i,j}\frac{b}{1+b}\\
    &= 1- \frac{b}{1+b}\sum_{i'\le i}w_{i',j} \tag{By telescoping the above recursion.}\\
    &\ge 1 - \frac{b}{1+b}\sum_{i'\in [n]}w_{i',j}\\
    &\ge 1 - \frac{b}{1+b} = \frac{1}{1+b} \tag{By applying our $P_{\Fcal}$ constraint.}
\end{align*}
Thus $p_{i,j}(v_i) \le 1$ so it is a valid probability. Notice that bidder $i$ receives item $j$ when he is not skipped and chooses menu
item $v_i$ with probability $x_{i,j}\frac{1}{(1+b)x_{i,j}}\pi_{i,j}(v_i) = \frac{1}{1+b}\pi_{i,j}(v_i)$. Thus we have a $(b, \frac{1}{1+b})$-selectable mechanism for any $b \in [0,1]$. By choosing $b=1$ we can see that our mechanism is a 2-approximation to the optimal BIC mechanism for this setting.


\subsubsection{Matching Constraints.}


Our ex-ante polytope $P_{\Fcal}$ can be fully described by the following constraints $\forall j \in [m]: \sum_{i \in [n]} w_{i,j} \le 1$, $\forall i \in [n]: \sum_{j \in [m]} w_{i,j} \le 1$. Again we will have $\Fcal_1 = \Fcal$ and $\lambda_1=1$. Let $A_{i,j}$ be the event that item $j$ is still available at bidder $i$'s turn. Lets call $x_{i,j} = \PP[A_{i,j}]$. Also, $B_{i,j}(v_i)$ be the event that no item $j'<j$ was allocated to bidder $i$ when items are considered sequentially, given that he was not skipped and given his type is $v_i$. Lets call $y_{i,j}(v_i) = \PP[B_{i,j}(v_i)]$. We will compute $x_{i,j}$, $y_{i,j}(v_i)$. As our base case we have that $\forall j \in [m], x_{1,j}=1$ and $\forall i \in [n], v_i \in \Vcal_i, y_{i,1}=1$. We are going to set $p_{i,j}(v_i) = \frac{p}{ x_{i,j} \cdot y_{i,j}(v_i)}$ where $p = \frac{2+b-\sqrt{b^2+4}}{2b}$ (we will later show that this is indeed a valid probability). Thus for bidder $1$ we are going to add elements $(1,1)$ with probability $p \pi_{1,1}(v_i)$. It is not difficult to see that: 

\begin{align*}
    y_{i,j+1}(v_i) &= y_{i,j}(v_i)\left((1-\pi_{i,j}(v_i)) +\pi_{i,j}(v_i)(1-x_{i,j})+\pi_{i,j}(v_i)x_{i,j}\left(1-\frac{p}{x_{i,j}y_{i,j}(v_i)}\right)\right)\\
    &= y_{i,j}(v_i)\left(1-\frac{\pi_{i,j}(v_i)p}{y_{i,j}(v_i)}\right)\\
    &= y_{i,j}(v_i) - p\pi_{i,j}(v_i)\\
    &= 1 - p\sum_{j'\le j}\pi_{i,j'}(v_i) \tag{Telescoping}\\
    &\ge 1-p \tag{Constraints}
\end{align*}
 Regarding the probability $x_{i+1,j}$ we can see that:

\begin{align*}
    &x_{i,j+1} \\
    &= x_{i,j}\left(1-b + b(1-y_{i,j})+b\sum_{v_i \in \Vcal_i} \PP[v_i]y_{i,j}(v_i)(1-\pi_{i,j}(v_i))+b\sum_{v_i \in \Vcal_i} \PP[v_i]y_{i,j}(v_i)\pi_{i,j}(v_i)\left(1-\frac{p}{x_{i,j}y_{i,j}(v_i)}\right) \right)\\
    &= x_{i,j} \left(1-\frac{w_{i,j}bp}{x_{i,j}}\right)\\
    &= x_{i,j} - bpw_{i,j}\\
    &= 1 - bp\sum_{i'\le i}w_{i,j} \tag{Telescoping}\\
    &\ge 1 - bp \tag{Constraints}
\end{align*}
By combining the two inequalities we have that:

\begin{align*}
    p_{i,j}(v_i) &= \frac{p}{ x_{i,j} \cdot y_{i,j}(v_i)}\\
    &\le \frac{p}{ (1-p)(1-bp)} \\
    &= \frac{\frac{2+b-\sqrt{b^2+4}}{2b}}{\left(1-\frac{2+b-\sqrt{b^2+4}}{2b}\right)\left(1- \frac{2+b-\sqrt{b^2+4}}{2}\right)} \\
    &= \frac{4+2b-2\sqrt{b^2+4}}{(b-2+\sqrt{b^2+4})(-b^2+\sqrt{b+4})}\\
    &= \frac{4+2b-2\sqrt{b^2+4}}{-b^2+b\sqrt{b^2+4}+2b-2\sqrt{b^2+4}-b\sqrt{b^2+4}+b^2+4}\\
    &= \frac{4+2b-2\sqrt{b^2+4}}{4+2b-2\sqrt{b^2+4}} =1
\end{align*}

 Thus $p_{i,j}(v_i)$ is a valid probability. Notice that from the perspective of bidder $i$, he receives item $j$ when he is not skipped and chooses menu item $v_i$ with probability $x_{i,j}y_{i,j}(v_i)\frac{p}{x_{i,j}y_{i,j}(v_i)}\pi_{i,j}(v_i)=p\pi_{i,j}(v_i)$. Thus we have a $(b,\frac{2+b-\sqrt{b^2+4}}{2b})$-selectable mechanism in this setting. By choosing $b=1$ we see that our mechanism is a $2-\phi$ approximation to the optimal mechanism where $\phi$ is the golden ratio.


\subsubsection{Knapsack Constraints.}
\label{section:knapsack}



Define for every item $j \in [m]$ some weight $d_j$. Our constraint now is that the total weight of items sold cannot be greater than $D$. Thus our ex-ante polytope $P_{\Fcal}$ can be fully described by the following constraint $\sum_{i \in [n]} \sum_{j \in [m]} w_{i,j} \cdot d_j \le D$. We will have $k=2$ with $\Fcal_1$ being the feasible set that only includes items with weight  $d_j>D/2$ and $\Fcal_2$ being the feasible set that only includes items with weight $d_j \le D/2$. We will run the heavy scheme with probability $\lambda_1 = \frac{1}{2}$ (Thus $\lambda_2 = 1 -\lambda_1 = \frac{1}{2}$). Let $S_h = \{j \in [m]: d_j>D/2\}$. 
Let $A_{i,j}(v_i)$ be the event that no item has been allocated until item $j \in S_h$ is considered at bidder $i$'s turn, given we run the heavy scheme and bidder $i$ chose menu item $v_i$. Lets call $x_{i,j}(v_i) = \PP[A_{i,j}(v_i)]$. We will compute $x_{i,j}(v_i)$ inductively. Disregard for now all items that are not in $S_h$. As our base case we have that $x_{1,1}=1$. We are going to have $p_{i,j}(v_i) = \frac{1}{(3+2b)x_{i,j}(v_i)}$ (we will later show that this is indeed a valid probability). It is not difficult to see that for $j\ge1$:

\begin{align*}
x_{i,j+1}(v_i) &= x_{i,j}(v_i)\cdot\left((1-\pi_{i,j}(v_i))+\pi_{i,j}(v_i)\left(1-\frac{1}{(3+2b)x_{i,j}(v_i)}\right) \right)\\
    &= x_{i,j}(v_i) \cdot \left(1-\pi_{i,j}(v_i)\frac{1}{(3+2b)x_{i,j}(v_i)} \right)\\
    &= x_{i,j}(v_i) - \frac{1}{3+2b}\pi_{i,j}(v_i) \\
    &= x_{i,1}(v_i) - \frac{1}{3+2b}\sum_{j' \in S_h: j' \le j} \pi_{i,j'}(v_i)
\end{align*}

Now lets compute $x_{i,1}$. It is not difficult to see that for $i\ge1$:

\begin{align*}
    x_{i+1,1}(v_{i+1}) &= \sum_{v_i \in \Vcal_i} \PP[v_i] x_{i,1}(v_i)\left(1-b + b\left(\frac{x_{i,1}(v_i)-\frac{1}{3+2b}\sum_{j' \in S_h}\pi_{i,j}(v_i)}{x_{i,1}(v_i)}\right)\right)\\
    &=\sum_{v_i \in \Vcal_i} \PP[v_i] x_{i,1}(v_i)\left(1-b + b\left(1-\frac{1}{(3+2b)x_{i,1}(v_i)}\sum_{j' \in S_h}\pi_{i,j}(v_i)\right)\right)\\
    &= x_{i,1}\left(1-\frac{b}{(3+2b)x_{i,1}}\sum_{j' \in S_h} w_{i,j'}\right)\tag{$x_{i,1}(v_i)$ invariant of $v_i$}\\
    &= x_{i,1} -\frac{b}{(3+2b)}\sum_{j' \in S_h}w_{i,j'} \\
    &= 1-\frac{b}{(3+2b)}\sum_{i'\le i}\sum_{j' \in S_h}w_{i',j'}
\end{align*}
Thus:
\begin{align*}
    x_{i,j}(v_i) &= 1-\frac{b}{(3+2b)}\sum_{i'< i}\sum_{j' \in S_h}w_{i',j'} - \frac{1}{(3+2b)}\sum_{j' \in S_h:j'<j} \pi_{i,j'}(v_i)\\
    &> 1-\frac{2b}{(3+2b)}-\frac{2}{(3+2b)} \tag{Given constraints and definition of $S_h$}\\
    &=\frac{1}{3+2b}
\end{align*}
It is not difficult to see that $p_{i,j}(v_i)\le 1$ for all $b \in [0,1]$. Thus given that we are using the heavy scheme bidder $i$ will receive item $j$ with probability $\frac{1}{3+2b}\pi_{i,j}(v_i)$ if he chooses menu item $v_i$. 

Now consider the light case.  Once a bidder is approached and he chooses a menu item $v_i$ for each item sequentially we will flip the two coins $\pi_{i,j}(v_i)$ and $p_{i,j}(v_i)$ and if both are 1 we will greedily allocate the item as long as the total weight of allocated items up until that point is no more than $\frac{D}{2}$. Let $B_{i,j}(v_i)$ be exactly that event and $y_{i,j}(v_i) = \PP[B_{i,j}(v_i)]$. Then we will set $p_{i,j}(v_i) = \frac{1}{(3+2b) \cdot y_{i,j}(v_i)}$. We discuss how to efficiently sample from $\frac{1}{(3+2b) \cdot y_{i,j}(v_i)}$ in \cref{section:efficient}. Let $D_{i,j}(v_i)$ be the expected weight of items sold up until pair $(i,j)$ is considered, given that bidder $i$ chose menu item $v_i$. Due to linearity of expectations we have that:

\begin{align*}
    \Ex{D_{i,j}(v_i)} &= \sum_{i'<i} \sum_{v_{i'} \in \Vcal} \sum_{j' \in [m]} b \frac{1}{(3+2b) \cdot y_{i',j'}(v_{i'})} y_{i',j'}(v_{i'}) \pi_{i',j'}(v_{i'}) d_{j'} + \sum_{j'<j} \frac{1}{(3+2b) \cdot y_{i',j'}(v_{i'})} y_{i',j'}(v_{i'}) \pi_{i',j'}(v_{i'}) d_{j'}\\
    &= \sum_{i'<i} \sum_{j' \in [m]} b \frac{1}{(3+2b)} w_{i',j'} d_{j'} + \sum_{j'<j} \frac{1}{(3+2b)} \pi_{i',j'}(v_{i'}) d_{j'} \\
    &\le \frac{b+1}{3+2b}D \tag{Due to constraints}
\end{align*}
Thus from Markov's inequality we have that:
\begin{align*}
    \PP[B_{i,j}(v_i)] &= \PP[D_{i,j}(v_i) < D/2] \\
    &= 1-\PP[D_{i,j}(v_i) \ge D/2] \\
    &\ge 1 - \frac{\frac{b+1}{3+2b}D}{D/2} \tag{Markov's Inequality}\\
    &= \frac{1}{3+2b}
\end{align*}
Thus $p_{i,j}(v_i)$ is a valid probability. Thus finally, bidders receive each item with a probability of $\frac{1}{6+4b}\pi_{i,j}(v_i)$ (We are losing an extra $1/2$ factor because we are running each scheme with probability $1/2$). Thus we have a $(b,\frac{1}{6+4b})$-selectable mechanism. By choosing $b=1$ we get a $1/10$-approximation for the knapsack constraints.


\subsubsection{Matroid Constraints.}

No consider that we have a total of $m + n$ different matroid constraints. For each item $j \in [m]$ we will have a matroid $M_j = (N_j, F_j)$ where $N_j = \{(i',j)\}_{i' \in [n]}$ is the universe of the matroid $M_j$. We shall call these per item constraints, horizontal. Also for each bidder $i$ we will have a matroid  $M^i = (N^i, F^i)$ where $N^i = \{(i,j')\}_{j' \in [m]}$ is the universe of the matroid $M^i$. We shall call these per bidder constraints, vertical. Here we will show how to do only horizontal or vertical constraints and in the next section we will show how to combine arbitrary downwards closed horizontal and vertical constraints.

\paragraph{Vertical Constraints}

Lets begin with the easier vertical constraints. From \cite{Feldman2021OCRS} we know that for any matroid there exists a $(b',1-b')$-selectable OCRS (different than our definition of selectable). Now since the constraint are per bidder then every menu item has to respect them. Then we will use the OCRS procedure described in \cite{Feldman2021OCRS} will result in a procedure where each item $j$ is allocated to $i$ with probability at least $b'(1-b')\pi_{i,j}(v_i)$. Thus we can adjust the coin flips $p$ so that it becomes exact. They key reason why we can readily black box OCRS results is that each item is selected independently with some probability and then greedily allocated.

\paragraph{Horizontal Constraints}

Again we will black box the OCRS results of \cite{Feldman2021OCRS}. Again from the perspective of bidder $i$ for item $j$ each of the pairs $(i',j), i'<i$ become independently active with probability $\sum_{v_{i'}} \PP[v_{i'}]p_{i',j}(v_i)\pi_{i',j}(v_i)$ and then greedily allocated if that did not conflict with the matroid constraint. Thus using the OCRS scheme of \cite{Feldman2021OCRS} and since each bidder is not skipped with probability $b$, each item can be selected with by bidder $i$ without any conflicts with the matroid constraints with probability at least $1-b$, thus he receives the item with probability at least $(1-b)\pi_{i,j}(v_i)$. Thus we can adjust the coin flips $p$ so that it becomes exact.


\subsubsection{Combining Constraints.}

The cases of combining horizontal with horizontal and vertical with vertical constraints is a simple extension of combining OCRS constraints of \cite{Feldman2021OCRS} so we will consider how we can combine a set of horizontal with a set of vertical constraints that presents some non-trivial difficulties. Also our approach work for any downwards closed vertical and horizontal constraints, not just matroids.

\paragraph{Vertical with Horizontal}. Conceptually we are going to run our or procedure two times once as if the horizontal constraints did not exist and once as if the vertical constraints do not exist. Between the two experiments we are going to couple the coin flips $\pi$ to be the same. We are going to allocate an item $j$ to bidder $i$ only if it has been allocate in both experiments. First notice that this procedure can be done online. It is just easier to conceptualize when we run the two experiments one after the other. Assume that the coin flips $\pi$ are both 1. The item will be allocated in the firs experiment with probability $c$ and in the second experiment with probability $c'$ due to the randomness of the allocation of the rest of the items. The important observation is that these events are independent. If one item ``passes'' the horizontal constraints does not affect the probability that it passes the vertical constraints due. Thus the probability that he finally receives the item with this procedure is exactly $c \cdot c' \cdot \pi_{i,j}$ . Now if we have a lower bound on $c$ and $c'$ for all pairs of items and bidders then we can construct appropriate coin flips to make the probability reduction exact. 

\paragraph{Arbitrary} Simple application of Union Bound.

\subsubsection{Efficient implementation considerations.}
\label{section:efficient}

In \cite{wrap157145} there is a description of a Bernoulli factory for division.

\subsection{Bidders with arbitrary utilities}

Let $\Scal$ be a set that contains all possible sets of items a bidder can receive. And suppose that for each bidder $i \in [n]$ we have a valuation function $u_{i}(\cdot,\cdot)$ that given as input a set $s \in \Scal$ and a payment $p\in \R$, outputs the utility of the bidder. We impose no constraints on $u_{i}(\cdot, \cdot)$. We allow for randomized allocations. Let $S$ be a probability distribution over sets in $\Scal$ and $P$ be a vector of payments where $p_s \in P$ is the payment when $s \in \Scal$ is sampled from $S$. Then $u_{i}(S, P) = \EX{s \sim S}{u_{i}(s, p_s)}$ depict the utility of bidder $i$ for that lottery. We assume that if a bidder gets nothing and pays nothing then his utility is zero (i.e. $u_i(\varnothing,0)=0$). 

We will extend our knapsack result to this setting. We will again assume that each item $j \in [m]$ has some weight $d_j$ and the sum of weights of allocated items cannot be greater than $D$. Obviously in this case there exist no $s \in \Scal$ such that $\sum_{j \in s} d_j > D$. Now assume that we have access to an interim allocation rule that maximizes the following non-convex LP:

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{i \in [n]} \displaystyle\sum\limits_{u_i \in \Ucal_i} \PP[u_i] \sum_{s \in \Scal} \pi_{i,s}(u_i) q_{i,s}(v_i)\\
\\
\text{s.t.}& \sum_{s \in \Scal} \pi_{i,s}(u_i) u_i(s,q_{i,s}(u_i)) &\ge \sum_{s \in \Scal} \pi_{i,s}(u'_i) u_i(s,q_{i,s}(u'_i)) & \forall i\in [n], u_i, u'_i \in \Ucal_i\\  
\\
&  \sum_{s \in \Scal} \pi_{i,s}(u_i) u_i(s,q_{i,s}(v_i)) &\ge 0 & \forall i\in [n], u_i \in \Ucal_i  \\
\\
& \sum_{s \in \Scal} \pi_{i,s}(u_i) &\le 1 & \forall i\in [n], u_i \in \Ucal_i
\\
\\
& \sum_{i \in [n]} \sum_{u_i \in \Ucal_i} \PP[u_i] \sum_{s \in \Scal} \pi_{i,s}(u_i) \sum_{j \in s} d_j &\le D
\end{array}
\end{equation*}

We will run a procedure inspired by our Knapsack solution of \cref{section:knapsack}. With probability $\lambda = \frac{2(b+1)}{5+4b}$ we are going to run the light scheme, and with probability $1-\lambda = \frac{3+2b}{5+4b}$ we are going to run the heavy scheme. In both cases we will consider bundles, bidder pairs sequentially and if we decide to allocate a bundle $s \in \Scal$ to bidder $i$ when he chose menu item $u_i$ we will charge him $q_{i,s}(u_i)$.

Lets first discuss the heavy scheme. In this case we are only going to consider bundles that have weight greater than half the total knapsack weight ($\Scal_h = \{s \in \Scal: \sum_{j \in s} d_j > \frac{D}{2}\}$). Obviously we can allocate such a bundle only to one bidder. Let $A_{i,s}(u_i)$ be the event that no item has been allocated until item $s \in \Scal_h$ is considered at bidder $i$'s turn, given we run the heavy scheme and bidder $i$ chose menu item $u_i$. Lets call $x_{i,s}(u_i) = \PP[A_{i,s}(u_i)]$. We can compute $x_{i,s}(v_i)$ inductively exactly the same way as we did in \cref{section:knapsack}. We are going to have $p_{i,s}(v_i) = \frac{1}{(3+2b)x_{i,s}(v_i)}$. The analysis of \cref{section:knapsack} shows that this is a valid probability. Thus, the probability with which a bidder is allocated a specific bundle $s \in \Scal_h$ and pays $q_{i,s}(u_i)$ is $(1-\lambda) x_{i,s}(u_i) \frac{1}{(3+2b)x_{i,s}(u_i)} \pi_{i,s}(u_i) = \frac{1}{5+4b}\pi_{i,s}(u_i)$.

Now lets consider the light scheme were we only take into account bundles in $\Scal_l = \{s \in \Scal: \sum_{j \in s} d_j \le \frac{D}{2}\}$. We are going to allocate a bundle to a bidder only if the items allocated up until that moment have weight less or equal to $D/2$.Let $B_i$ be the event that the items allocated up until bidder $i$ have weight less or equal to $D/2$. Lets call $y_i = \PP[B_i]$. Also let $C_{i,s}(u_i)$ be the event that when bidder $i$ chooses menu item $u_i$ there have not been any bundles allocated to that bidder before bundle $s$ is considered. Let $z_{i,s}(u_i) = \PP[C_{i,s}(u_i)]$. We will consider each bundle sequentially and we will flip two coins, one with probability $\pi_{i, s}(u_i)$ and one with probability $p_{i,s}(u_i) = \frac{1}{2(b+1)y_i z_{i,s}(u_i)}$. If both turn out to be 1 and the total weight of items allocated until that point is less or equal to $D/2$ and no other bundle is allocated to that bidder then we give him that bundle. Thus, the probability with which a bidder is allocated a specific bundle $s \in \Scal_l$ and pays $q_{i,s}(u_i)$ is $\lambda y_i z_{i,s}(v_i) \frac{1}{2(1+b)y_i z_{i,s}(u_i)} \pi_{i,s}(u_i) = \frac{1}{5+4b}\pi_{i,s}(u_i)$. The only thing left to show is that $\frac{1}{2(b+1)y_i z_{i,s}(u_i)}$ is a valid probability. First it is not hard to see that:

\begin{align*}
    z_{i,s+1}(u_i) &= z_{i,s}(u_i)\left(1-\frac{1}{2(1+b)y_i z_{i,s}(u_i)}\pi_{i,s}(u_i)\right)\\
    &= z_{i,s}(u_i) - \frac{1}{2(1+b)y_i}\pi_{i,s}(u_i)\\
    &= 1 - \frac{1}{2(1+b)y_i} \sum_{s'\le s} \pi_{i,s}(u_i)\\
    &\ge 1- \frac{1}{2(1+b)y_i}
\end{align*}
Thus we have that $p_{i,s}(u_i) \le \frac{1}{2(b+1)y_i- 1}$. Now lets focus on $y_i$. Lets call $D_i$ the random variable that represents the weight of items allocated until bidder $i$'s turn. Due to linearity of expectation ,we have that:
\begin{align*}
    \Ex{D_i} &= \sum_{i'<i} \sum_{u_i \in \Ucal_i} \sum_{s \in \Scal_l} b \PP[u_i] y_i z_{i,s}(u_i) \frac{1}{2(b+1)y_i z_{i,s}(u_i)} \pi_{i,s}(u_i) d_j \\
    &= \sum_{i'<i} \sum_{u_i \in \Ucal_i} \sum_{s \in \Scal_l} \PP[u_i]  \frac{b}{2(b+1)} \pi_{i,s}(u_i) d_j \\
    &\le \frac{b}{2(b+1)}D
\end{align*}
Thus from a simple application of Markov's inequality we get that $\PP[B_i]\ge \frac{1}{1+b}$. Thus $p_{i,s}(u_i) \le \frac{1}{\frac{2(b+1)}{b+1}- 1} = 1$. Thus we have a $(b,\frac{1}{5+4b})$-selectable mechanism for this setting. By choosing $b=1$ we get a $\frac{1}{9}$-approximation to the optimal revenue in this setting.


\subsubsection{Quasi-Linear Bidders}

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{i \in [n]} \displaystyle\sum\limits_{v_i \in \Vcal_i} \PP[v_i] q_i(v_i)\\
\\
\text{s.t.}& \sum_{s \in \Scal} v_{i}(s)\pi_{i,s}(v_i) - q_i(v_i) &\ge \sum_{s \in \Scal} v_{i}(s)\pi_{i,s}(v'_i) - q_i(v'_i) & \forall i\in [n], v_i, v'_i \in \Vcal_i\\  
\\
&  \sum_{s \in \Scal} v_{i}(s)\pi_{i,s}(v_i) - q_i(v_i) &\ge 0 & \forall i\in [n], v_i \in \Vcal_i  \\
& \sum_{s \in \Scal} \pi_{i,s}(v_i) &\le 1 & \forall i\in [n]
\\
\\
& \sum_{i \in [n]}\sum_{s \in \Scal} \pi_{i,s}(v_i) \sum_{j \in s} d_j &\le D
\end{array}
\end{equation*}

The above LP can be solved in polynomial time to $|\Scal|, |\Vcal|$, and $n$.

Using the intuition of the previous sections we can easily see how given an interim allocation rule we can transform it to an online ex-post feasible mechanism.

\section{Procurement Auctions}

We now assume that the designer is the buyer and the participants in the mechanism are the sellers. Each seller has a total of $m$ services. For each seller $i \in [n]$ and service $j \in [m]$, the buyer has some known value $v_{i,j}$. The buyer wants to maximize his total acquired value by buying services without surpassing his hard budget $B$. Each seller $i \in [n]$ has some cost for providing service $j \in [m]$ depicted as $c_{i,j}$. We will assume that $c_i$ is drawn from some known distribution $\Ccal_i$. We can write the following LP that solve a relaxations of our problem:

\begin{equation*}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{i \in [n]} \displaystyle\sum\limits_{c_i \in \Ccal_i} \PP[c_i] \sum_{j \in [m]} \pi_{i,j}(c_i) v_{i,j}\\
\\
\text{s.t.}&  q_i(c_i) - \sum_{j \in [m]} c_{i,j} \pi_{i,j}(c_{i}) &\ge q_i(c'_i) - \sum_{j \in [m]} c_{i,j} \pi_{i,j}(c'_{i}) & \forall i\in [n], c_i, c'_i \in \Ccal_i\\  
\\
&  q_i(c_i) - \sum_{j \in [m]} c_{i,j} \pi_{i,j}(c_{i}) &\ge 0 & \forall i\in [n], v_i \in \Vcal_i  \\
\\
& \sum_{i \in [n]} \sum_{c_i \in \Ccal_i} \PP[c_i] q_i(c_i) &\le B 
\\
\\
& q_i(c_i) \le B
\end{array}
\end{equation*}

We are going to use ideas similar to the ones of the previous sections. Assume we have the solution to the above LP which is a relaxation of the problem we seek to solve.

We are going to approach each seller sequentially and ask them their costs. Based on their response we are going to pay them $q_i(c_i)$ with some probability $\alpha$ otherwise we are going to pay them $0$. From that seller we are going to take a randomized set of services where each service is taken with probability $c \pi_{i,j}(c_i)$. The mechanism is incentive compatible and interim IR (we can make it ex-post IR with some extra tricks).

We are going to approach sellers sequentially. Each seller will be considered with probability $b$ or skipped with probability $1-b$. With probability $1/2$ we are going to run the big scheme and with probability $1/2$ we are going to run the small scheme.

When we run the big scheme we are only going to pay the bidders who tell us a cost $c_i$ such that the interim payment $q_i(c_i) > \frac{1}{2}B$. Let $\Ccal^B_i = \{c_i \in \Ccal_i:q_i(c_i) > \frac{1}{2}B \}$. When a seller arrives and reports costs $c_i$ such that $q_i(c_i) > \frac{1}{2}B$ we flip a coin $p_{i}$ with probability $\frac{1}{(2b+1) x_i}$ where $x_i$ is the probability that we have not paid any other seller up until that point. Once we flip that coin and we have not paid any other seller up until that point we pay him $q_i(c_i)$. Thus the expected payment is equal to $\frac{1}{2b+1}q_i(c_i)$. Now lets calculate $x_i$ to show that $p_i$ is a valid coin:

\begin{align*}
    x_{i+1} &= x_{i}\left(1-b + b (1-p_i)+ bp_i\left(1-\sum_{c_{i} \in \Ccal^B_{i}} \PP[c_{i}]\right)\right)\\
    &= x_{i}\left(1- bp_i \sum_{c_{i} \in \Ccal^B_{i}} \PP[c_{i}] \right)\\
    &= x_i -\frac{b}{2b+1}\sum_{c_{i} \in \Ccal^B_{i}} \PP[c_{i}]\\
    &= 1-\frac{b}{2b+1} \sum_{i' \le i} \sum_{c_{i'} \in \Ccal^B_{i'}} \PP[c_{i'}]\\
    &\ge 1-\frac{2b}{2b+1} = \frac{1}{2b+1}
\end{align*}
Which proves that $p_i$ is a valid coin. Thus overall if a seller reports costs $c_i \in \Ccal^B_{i}$ he is going to be paid with a $\frac{1}{4b+2}$ probability.

If we run the small scheme we are only going to pay sellers that report costs $c_i$ such that the interim payment $q_i(c_i) \le \frac{1}{2}B$. Let $\Ccal^S_i = \{c_i \in \Ccal_i:q_i(c_i) \le  \frac{1}{2}B \}$. When a seller arrives and reports costs $c_i$ such that $q_i(c_i) \le \frac{1}{2}B$ we flip a coin $p_{i}$ with probability $\frac{1}{(2b+1) y_i}$ where $y_i$ is the probability that we have not paid a total of more than $\frac{1}{2}B$ up until that point. Once we flip that coin and we have not exhausted more than half our budget up until that point we pay him $q_i(c_i)$. Thus the expected payment is equal to $\frac{1}{2b+1}q_i(c_i)$. Now lets calculate a lower bound on $y_i$ to show that $p_i$ is a valid coin. Let $D_i$ be the random variable that represents the total amount we have paid to sellers until the $i^{th}$ sellers turn. Due to linearity of expectation we have that:

\begin{align*}
    \Ex{D_i} &= \sum_{i' < i} \sum_{c_{i'} \in \Ccal^S_{i'}} b p_{i'} y_{i'} \PP[c_{i}] q_{i'}(c_{i'})\\ 
    &= \sum_{i' < i} \sum_{c_{i'} \in \Ccal^S_{i'}} \frac{b}{2b+1}\PP[c_{i}] q_{i'}(c_{i'})\\
    &\le \frac{b}{2b+1} B
\end{align*}
Now by applying Markov's inequality we get that $y_i \ge \frac{1}{2b+1}$. By choosing $b=1$ we see that our mechanism is a $\frac{1}{6}$-approximation to the optimal procurement auction.

Given the stochastic knapasck OCRS of \cite{jiang2022tight} we can actually get a $\frac{1}{3+e^{-1}}$ approximation.



\section{Questions}
\begin{enumerate}
    \item Given an OCRS for constraint X, can we get an ex-interim mechanism for constraint X?
        \begin{itemize}
            \item If the constraints are of the form ``per agent'' or ``per item'' or intersections then yes.
        \end{itemize}
    \item Given lower bounds for OCRSs, do we get lower bounds for the ex-interim approach? Equivalently, given an ex-interim mechanism, do we get an OCRS?
        \begin{itemize}
            \item If the constraints are of the form ``per agent'' or ``per item'' or intersections then yes.
        \end{itemize}
    \item Is there a connection between Alaei's simultaneous setting an CRS? Anything we can improve (given modern CRS)?
\end{enumerate}


